Extreme Treatment Effect: Extrapolating Dose-Response Function Into Extreme Treatment Domain

The potential outcomes framework serves as a fundamental tool for quantifying causal effects. The average dose-response function (also called the effect curve), denoted as (\mu(t)), is typically of interest when dealing with a continuous treatment variable (exposure). The focus of this work is to determine the impact of an extreme level of treatment, potentially beyond the range of observed values--that is, estimating (\mu(t)) for very large (t). Our approach is grounded in the field of statistics known as extreme value theory. We outline key assumptions for the identifiability of the extreme treatment effect. Additionally, we present a novel and consistent estimation procedure that can potentially reduce the dimension of the confounders to at most 3. This is a significant result since typically, the estimation of (\mu(t)) is very challenging due to high-dimensional confounders. In practical applications, our framework proves valuable when assessing the effects of scenarios such as drug overdoses, extreme river discharges, or extremely high temperatures on a variable of interest.

==> sections/Discarded.tex <==
Under Assumptions  \ref{assumption_max_domain}, \ref{assumption_unconfoundness_tail}  and \ref{assumption_linearity_of_tail_1} and Assumption C, we know that $\mu_{\textbf{x}}(t) \sim \alpha{\tau}_{lin}^\top\textbf{x} + \beta{\tau}_{lin}^\top\textbf{x}t$ as $t\to\tau_R$ (see Lemma~\ref{lemma2}) and hence, ${\omega}_{\textbf{x}^\star} = \beta \tau_{lin}^\top\textbf{x}^\star$. We will show that our estimators of $\hat{\beta}$ and $\hat{\tau}_{lin}$ are consistent. If we manage to show that, Slutsky`s theorem give us that $\hat{\omega}_{\textbf{x}^\star}$ is consistent. 

Note that a model
\begin{equation}\label{model_asymptot}
    \mathbb{E}[Y\mid T=t, \textbf{X}=\textbf{x}] = \alpha{\tau}_{lin}^\top\textbf{x} + \beta{\tau}_{lin}^\top\textbf{x}t
\end{equation}
is valid only asymptotically (for $t\approx \tau_R$). Hence, for any given $\varepsilon$, it is possible to find $t_0$ such that for all $t>t_0$ and for all $\textbf{x}\in\mathcal{X}$ holds 


$$1-\varepsilon<\frac{\mathbb{E}[Y\mid T=t, \textbf{X}=\textbf{x}]}{ \alpha{\tau}_{lin}^\top\textbf{x} + \beta{\tau}_{lin}^\top\textbf{x}t}<1+\varepsilon.$$


Fix $t>t_0$ and find $n_0\in\mathbb{N}$ such that for all $\textbf{x}$ holds $t<F^{-1}_{T\mid \textbf{X} = \textbf{x}}(q_{n_0})$; in other words, $q_{n_0}$ is large enough such that the  $q_{n_0}$-quantile of $T\mid\textbf{X}$ is larger than $t$. Hence, we can assume an exact validity of (\ref{model_asymptot}) and our estimation will be imprecise up to a factor of $\varepsilon$. We neglige this imprecisity by sending $\varepsilon\to 0$. 

Now we focus on consistency of $\hat{\tau}_{lin}$. It is well known that for a fixed quantile $q$, the maximum likelihood estimator $\hat{\tau}_{lin} = argmin_b\sum_{i=1}^nh_q(T_i - \textbf{X}_i^\top b)$ is consistent and even asymptotically normal (see e.g. Theorem 4.1 in \cite{koenker_2005}, noting that we assume continuous $T$ and finite second moments of $\textbf{X}$). However, quantile $q$ is not fixed and is increasing with the sample size with the speed  $\lim_{n\to\infty}q_n=1$ and $\lim_{n\to\infty}n(1-q_n)=\infty$. This is a well-known generalization of quantile regression known as 'intermediate order regression quantiles' or 'moderately extreme quantiles' \citep{chernozhukov2016extremal} and is as well consistent and asymptotically normal under Assumption~C (see Theorem 5.1 in \cite{chernozhukov2005extremal}). 

Next, we show that $\hat{\beta}$ is consistent estimator of $\beta$. For now, fix $\tau_{lin}\neq \textbf{0}$. It is an elementary knowledge that the estimation of $\beta$ using least squares in a model $$\mathbb{E}[Y\mid T=t, T>{\tau}_{lin}^\top\textbf{x}, \textbf{X}=\textbf{x}] = \alpha{\tau}_{lin}^\top\textbf{x} + \beta{\tau}_{lin}^\top\textbf{x}t,$$  where $\tau_{lin}$ is fixed, is consistent and even asymptotically normal under conditions $var(Y)<\infty$ ,  $\mathbb{E}||\textbf{X}||^2<\infty$, $(\textbf{X}, T$) satisfying Grenander conditions and the sample-size $|S|=:k_n = n(1-q_n)\to\infty$.    (see e.g. Lemma~\ref{lemma_grenander}). 

Note that least squares estimate $\hat{\beta}$ is linear in $\tau_{lin}$: that is, if we express  $\hat{\beta}$ explicitly, we get $\hat{\beta} = \tau_{lin}^\top \widehat{\tilde{\beta}}$, where   $\tilde{\beta}$ is a coefficient in a linear model corresponding to (\ref{ewqfdwef}). We finish the proof by replacing  $\tau_{lin}$ by its estimate $\hat{\tau}_{lin}$ and using one more time Slutsky`s theorem: since $\widehat{\tilde{\beta}}$ is consistent, we get also that $\hat{\tau}_{lin}^\top \widehat{\tilde{\beta}}$ is consistent and hence, $\hat{\beta}$ is consistent estimation of $\beta$.  

We present an an illustration of the linearity of  $\hat{\beta}$  in $\tau_{lin}$ for $d=1$.  An explicit expression of $\hat{\beta}$ as a function of $\tau_{lin}$ and our data explicitly is the following: 
\begin{equation}
\begin{bmatrix}
    \hat{\alpha} \\
    \hat{ \beta}
\end{bmatrix}
=
(M^\top M)^{-1}M^\top\textbf{Y}_S, \,\,\,\,\,\,\,\,where\,\,\,\,\, 
M=\begin{bmatrix}
    {\tau}_{lin}\textbf{x}_{1} &  {\tau}_{lin}\textbf{x}_{1}t_{1} \\ \dots &  \dots \\ {\tau}_{lin}\textbf{x}_{k}&  {\tau}_{lin}\textbf{x}_{k}t_{k} \\
\end{bmatrix}
\end{equation}
where $\textbf{Y}_S= (Y_1, \dots, Y_k)^\top$, WLOG let $S=\{1, \dots, k_n\}\subset\{1, \dots, n\}$.   Note that \begin{equation}
M =  {\tau}_{lin} diag(x_1, \dots, x_k)
\begin{bmatrix}
 1 & t_{1} \\ \dots &  \dots \\ 1&  t_{k} \\
\end{bmatrix}={\tau}_{lin} \tilde{M},
\end{equation}
where  $\tilde{M}$ is the data-matrix corresponding to a model (\ref{ewqfdwef}). 



We finish the proof by using Slutsky`s theorem again: Since  $\hat{\beta}$ and $\hat{\tau}_{lin}$ are consistent estimators, we also get that for a fixed $\textbf{x}^\star$ is $\hat{\omega}_{\textbf{x}^\star} = \hat{\beta}\hat{\tau}_{lin}^\top\textbf{x}^\star$ consistent. 

The weights are often inspired by the following observation \citep{huang2022extreme}: Given the unconfoundedness and positivity assumptions, any measurable function $\phi$ satisfies 
\begin{equation*}
    \begin{split}
        \mathbb{E}[\phi\{Y(t)\}] 
    &= \mathbb{E}(\mathbb{E}[\phi\{Y(t)\}\mid \textbf{X}]) = \mathbb{E}(\mathbb{E}[\phi\{Y(t)\}\mid \textbf{X}, T=t]) = \mathbb{E}(\mathbb{E}[\phi\{Y\}\mid \textbf{X}, T=t])           
   \\&=\int_{\mathcal{X}}\int_{\mathcal{Y}}\phi(y) p_{Y\mid \textbf{X}, T}(y, \textbf{x}, t)p_\textbf{X}(\textbf{x})dyd\textbf{x}
   \\&=\int_{\mathcal{X}}\int_{\mathcal{Y}}\phi(y) \frac{p_T(t)}{p_{T\mid \textbf{X}}(t\mid \textbf{x})} p_{Y, \textbf{X}\mid T}(y,\textbf{x}\mid t) dy d\textbf{x} 
   \\&=\mathbb{E}\{\pi_0(T, \textbf{X})\phi(Y)\mid T=t\}, \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\text{ where }\pi_0(t,x) := \frac{p_T(t)}{p_{T\mid \textbf{X}}(t\mid \textbf{x})}.
    \end{split}
\end{equation*}
Hence, modelling the weights $\pi_0(t,x)$ is a cornerstone for estimating the causal effect. 







\begin{lemma}
Under Assumptions~\ref{assumption_unconfoundness_tail}, \ref{assumption_positivity_tail} and \ref{assumption_max_domain} holds
\begin{equation}\label{eq1}
  \mathbb{E}[Y(t)\mid  \theta(\textbf{X})]\sim \mathbb{E}[Y\mid  T=t, \theta(\textbf{X})]\,\,\,\,\,\,\,\,\, \text{   for    }t\to\tau_R.  
\end{equation}
Hence, 
$$\mu(t) \sim \int \mathbb{E}[Y\mid  T=t, \theta(\textbf{x})]p_{\theta(\textbf{X})}(\textbf{x})d\textbf{x}\,\,\,\,\,\,\,\,\, \text{   for    }t\to\tau_R.$$
\end{lemma}
\begin{proof}
First, we show that 
\begin{equation}\label{eq35}
    p_{T\mid \textbf{X}, T>t} \overset{asym.}{=} p_{T\mid \theta(\textbf{X}), T>t}\,\,\,\,\,\,\,\,\, \text{   as    }t\to\tau_R.
\end{equation}
 This is trivial: Assumption~\ref{assumption_max_domain} implies that the distribution of $[T-t\mid T>t]$ approaches GPD distribution with some parameters $\theta\in\mathbb{R}^2$. Also, the distribution of $[T-t\mid T>t, \textbf{X}]$ approaches GPD distribution with parameters $\theta(\textbf{X})$. Hence, the distribution of $[T\mid T>t, \textbf{X}]$ is fully characterized by the parameters $\theta(\textbf{X})$ and is therefore equal to  the distribution of $[T\mid T>t, \theta(\textbf{X})]$. 

Next, we show 
\begin{equation}
  \label{eq2}
    p_{T, Y(t)\mid \theta(\textbf{X}), T>t} \overset{asym.}{=}  p_{T\mid \theta(\textbf{X}), T>t}p_{Y(t)\mid \theta(\textbf{X}), T>t}, \,\,\,\,\,\text{ as }t\to\tau_R.
  \end{equation}
  In order to prove (\ref{eq2}) consider the (trivial) equality 
\begin{equation}\label{eq3}
    p_{T, \textbf{X}, Y(t)\mid \theta(\textbf{X}), T>t} =  p_{T, \textbf{X}\mid \theta(\textbf{X}), T>t}  p_{Y(t)\mid \theta(\textbf{X}),  T,\textbf{X}, T>t}. 
\end{equation}
Denote by $LS$ the left side of (\ref{eq3}). Using (\ref{eq35}), we get $$
 p_{T, \textbf{X}\mid \theta(\textbf{X}), T>t} \overset{asym.}{=}  p_{T\mid \theta(\textbf{X}), T>t}p_{\textbf{X}\mid \theta(\textbf{X}), T>t}. 
  $$
  Hence,  (\ref{eq3}) satisfies 
  $$
LS \overset{asym.}{=} p_{T\mid \theta(\textbf{X}), T>t}\,\,p_{\textbf{X}\mid \theta(\textbf{X}), T>t}\,\,p_{Y(t)\mid \theta(\textbf{X}), T,\textbf{X},  T>t}
  $$

  Combining the final two terms of this expression and integrating over $\textbf{X}$, we obtain (\ref{eq2}). 
  
Finally, we are ready to prove (\ref{eq1}). We proceed by combining Assumption \ref{assumption_unconfoundness_tail} together with (\ref{eq35}). Since the following holds: 
$$\mathbb{E}[Y(t)\mid  \textbf{X}]\sim \mathbb{E}[Y\mid  T=t, \textbf{X}]\,\,\,\,\,\,\,\,\, \text{   as    }t\to\tau_R,$$
we condition on $\theta(\textbf{X})$ and integrate over the remaining $\textbf{X}$. Since integrating over $\textbf{X}$ will not affect $T$, we proved the claim. 
  


 The second equation trivially follows from the second by integrating over $\theta(\textbf{X})$. 
 \end{proof}








==> sections/Thoughts.tex <==

\subsection{Simulations with a high dimensional $\textbf{X}$}
\label{Section_simulations_hidden_confounder}
In this simulations we consider $\textbf{X} = (X_1, \dots, X_d)$ where the dimension $d$ is potentially large. Consider the following data-generating process:
\begin{itemize}
    \item Let $a_1, \dots, a_d\overset{iid}{\sim} \mathcal{N}(1,1)$ and $b_1, \dots, b_d\sim \mathcal{N}(-1,1)$ be fixed numbers at the beginning of the simulations. 
    \item Consider $\textbf{X}$ being centered Gaussian vector with $cor(X_i, X_j)=0.1$ for all $i\neq j$.
    \item Let $T = \sum_{i=1}^d a_iX_i + \varepsilon_T$, where $\varepsilon_T$ is distributed according to either $\mathcal{N}(0,10)$, $Exp(\frac{1}{10})$ or $Pareto(1,1)$. 
    \item Let $Y = \mu_{x}(T) +\sum_{i=1}^d b_iX_i + \varepsilon_Y $, where $\mu_x(t)$ is defined in (\ref{eq875}) with hyper-parameters $c=slope(x)=1$ and where $\varepsilon_Y\sim\mathcal{N}(0,1)$.
\end{itemize}

This data generating process leads to $\mu(t+1) - \mu(t) = -slope(x) = -1$ for $t\geq c$ and $ \mu(t+1) - \mu(t) = +1$ for $t<c$. Consequently, our primary interest lies in estimating $\omega = \mu(t+1) - \mu(t) =-1$ for $t\geq c$.

Note that a simple linear regression $Y\sim T + X_1 + \dots + X_d$ leads to a biased estimation of the effect of $T$, since the effect is different for large and for small values of $T$. However, simply discarding values where $T_i<1$ leads to a selection bias and hence, classical statistical methods do not apply here. 

We generate data as specified with a sample size of $n=5000$. Setting the threshold at $\tau = 0.95$, we employ the methodology outlined in Section~\ref{section_algorithm} to estimate $\omega$. Specifically, we utilize linear parametrization of the parameters in the estimation procedure. This process is repeated $100$ times. The mean of the estimates $\hat{\omega}$ together with $95\%$ quantile for various values of $d$ and distributions of the noise variables can be found in Table~\ref{table_simulations_dimension_d}.

Table~\ref{table_simulations_dimension_d} illustrates that with a sample size of $n=5000$, the results are reasonably accurate as long as $d\leq 50$. The reason for the bias observed in larger dimensions $d$ is that Assumption~\ref{assumption_max_domain} and (\ref{eq1}) are only asymptotic results, and with higher dimensions $d$, we require more data for the asymptotic theory for $T\mid \textbf{X}$ to take effect. It is well known that the convergence rate of the maxima of the Gaussian random sample to an extreme value distribution is very slow, whereas it is faster with Exponential or Pareto distribution \citep{Davis_convergence}. With a large dimension $d$, we also observe a more pronounced effect of the estimation error accumulated in the first step on the second step of the algorithm.
\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
True $\omega=-1$& Gaussian $\varepsilon_T$         & Exponential $\varepsilon_T$    & Pareto $\varepsilon_T$         \\ \hline
$d=5$       & $\hat{\omega} =-1.0 \pm 0.03$& $\hat{\omega} =-1.0 \pm 0.01$& $\hat{\omega} =-1.0 \pm 0.001$\\ \hline
$d=25$      & $\hat{\omega} =-0.96 \pm 0.08$   & $\hat{\omega} =-0.99 \pm 0.01$ & $\hat{\omega} =-1.0 \pm 0.001$\\ \hline
$d=50$      & $\hat{\omega} = -0.75 \pm 0.28 $ & $\hat{\omega} =-0.97 \pm 0.09$ & $\hat{\omega} =-0.99 \pm 0.01$ \\ \hline
$d=200$     & $\hat{\omega} = -0.44\pm 0.37 $  & $\hat{\omega} =-0.53 \pm 0.42$ & $\hat{\omega} =-0.91 \pm 0.68$\\ \hline
\end{tabular}
\caption{Estimates of $\omega=-1$ with varying dimension of the confounders $d=dim(X)$ and with different distributions of $T$. Note that the sample size in these simulations is $n=5000$.}
\label{table_simulations_dimension_d}
\end{table}





























